IlluSign: Illustrating Sign Language Videos by Leveraging the Attention Mechanism

Sign languages are dynamic visual languages that involve hand gestures, in combination with non manual elements such as facial expressions. While video recordings of sign language are commonly used for education and documentation, the dynamic nature of signs can make it challenging to study them in detail, especially for new learners and educators. This work aims to convert sign language video footage into static illustrations, which serve as an additional educational resource to complement video content. This process is usually done by an artist, and is therefore quite costly. We propose a method that illustrates sign language videos by leveraging generative models' ability to understand both the semantic and geometric aspects of images. Our approach focuses on transferring a sketch like illustration style to video footage of sign language, combining the start and end frames of a sign into a single illustration, and using arrows to highlight the hand's direction and motion. While many style transfer methods address domain adaptation at varying levels of abstraction, applying a sketch like style to sign languages, especially for hand gestures and facial expressions, poses a significant challenge. To tackle this, we intervene in the denoising process of a diffusion model, injecting style as keys and values into high resolution attention layers, and fusing geometric information from the image and edges as queries. For the final illustration, we use the attention mechanism to combine the attention weights from both the start and end illustrations, resulting in a soft combination. Our method offers a cost effective solution for generating sign language illustrations at inference time, addressing the lack of such resources in educational materials.

==> figures/figure_1_final_overlay.tex <==

% Use figure* for multi-column figure
% \vspace*{\fill}
\begin{figure*}[htb]
    
    \centering
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/affe_final.png}
    \end{minipage}
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/beijing_final.png}
    \end{minipage}
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/bonn_final.png}
    \end{minipage}
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/drogen_final.png}
    \end{minipage}
    \begin{minipage}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/air_final.png}
    \end{minipage}

    \centering
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/fangrnframe_0014.jpg}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/fangenframe_0023.jpg}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/fangen_final.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/eltern_frame_0015.jpg}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intro/eltern_frame_0038.jpg}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/intro/eltern_final.png}
    \end{minipage}



    
    \caption{In this work we present a method for transforming images of sign language video frames into detailed illustrations which highly preserve the geometrical details in images, emphasizing hand gestures alongside hand direction and motion. For non occluding hands sequential frames we also show the option of combining the illustration into one final detailed illustration.}
    \label{fig:illustration}
\end{figure*}



==> figures/method_overlay.tex <==

\begin{figure}[t] %
    \centering
    \begin{subfigure}{0.32\columnwidth} % 
        \includegraphics[width=\linewidth]{figures/method_overlay/name_out_q1---seed_42.png}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/name_out_q2---seed_42.png}
        % \caption{B}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/name_out_transfer---seed_42.png}
        % \caption{C}
    \end{subfigure}

    % \vspace{5pt} % Adds vertical spacing between rows

    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_q1---seed_42.png}
        % \caption{D}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_q2---seed_42.png}
        % \caption{E}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_transfer---seed_42.png}
        % \caption{F}
    \end{subfigure}

    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/mensch_frame_0012.png}
        \centering
        \text{Start Illustration}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/mensch_frame_0023.png}
        % \caption{H}
        \centering
        \text{End Illustration}
    \end{subfigure}
    \begin{subfigure}{0.32\columnwidth}
        \includegraphics[width=\linewidth]{figures/method_overlay/mensch_queries_init_q1_q2.png}
        % \caption{I}
        \centering
        \text{Illustration Overlay}
    \end{subfigure}

    \caption{Composite overlay illustration, generated from start and end of sign illustrations.}
    \label{fig:grid_overlay}
\end{figure}



==> figures/method_style_transfer.tex <==

% \begin{figure}[t] %
%     \centering
%     \begin{subfigure}{0.32\columnwidth} % 
%         \includegraphics[width=\linewidth]{figures/method_overlay/name_out_q1---seed_42.png}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/name_out_q2---seed_42.png}
%         % \caption{B}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/name_out_transfer---seed_42.png}
%         % \caption{C}
%     \end{subfigure}
%     % \begin{subfigure}{0.32\columnwidth}
%     %     \includegraphics[width=\linewidth]{figures/method_overlay/name_out_transfer---seed_42.png}
%     %     % \caption{C}
%     % \end{subfigure}

%     % \vspace{5pt} % Adds vertical spacing between rows

%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_q1---seed_42.png}
%         % \caption{D}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_q2---seed_42.png}
%         % \caption{E}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/st_josephout_transfer---seed_42.png}
%         % \caption{F}
%     \end{subfigure}

%     % \vspace{5pt}

%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/mensch_frame_0012.png}
%         % \caption{G}
%         \text{Start Illustration}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/mensch_frame_0023.png}
%         % \caption{H}
%         \text{End Illustration}
%     \end{subfigure}
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\linewidth]{figures/method_overlay/mensch_queries_init_q1_q2.png}
%         % \caption{I}
%         \text{Final Illustration}
%     \end{subfigure}

%     \caption{Final overlay illustration, generated from start and end of sign illustrations.}
%     \label{fig:grid_style}
% \end{figure}


